DiaNet: BERT and Hierarchical Attention Multi-Task Learning of Fine-Grained Dialect

Prediction of language varieties and dialects is an important language processing task, with a wide range of applications. For Arabic, the native tongue of ~ 300 million people, most varieties remain unsupported. To ease this bottleneck, we present a very large scale dataset covering 319 cities from all 21 Arab countries. We introduce a hierarchical attention multi-task learning (HA-MTL) approach for dialect identification exploiting our data at the city, state, and country levels. We also evaluate use of BERT on the three tasks, comparing it to the MTL approach. We benchmark and release our data and models.

==> semi-supervised_exps.tex <==
\section{Semi-Supervised Models}

\subsection{Self-Training with Unlabeled Data}
We employ self-training, a type of semi-supervised learning where a model is trained on gold labeled data and is used to tag a large amount of unlabeled data, with a goal to augment the gold training set with the most `\textit{confidently}' predicted cases. In our neural network models, we use the per-class value in the softmax layer as a confidence threshold. In other words, we consider tweets predicted above a given threshold `\textit{good enough}' and we use them to augment our training set. We run our self-training on a pool of 10M tweets (we refer to this set simply as \texttt{unlabeled}). \mam{explain how we extract this pool.} We have two settings for self-training with unlabeled data, \textit{(a) class-agnostic} and \textit{(b) class-specific}. For (a) class-agnostic, we add the top confidently predicted percentage of \texttt{unlabeled}, irrespective of the class assigned to a data point, to gold train. We experiment with top percentages from the set \textit{\{5\%, 10\%, 25\%\}}. For 
(b) class-specific, we add the top confidently predicted cases assigned to each class, again with values from the set \textit{\{5\%, 10\%, 25\%\}}. The class-specific setting ensures we get enough data from classes where the model tends not to be as highly confident as other classes dominating the training set. Table~\ref{tab:ssl_res} provides our results for the self-training experiments. \mam{This table should spell out all res across all self-traing exps, from this and next section}.

 \mam{describe how we acquire data for self-training. Describe including only tweets > 30/40? words length, only in direct addresses/replies between users, and with zero diacritics. \textbf{Importantly}, we can analyze the softmax values in the validation set, to get a per-class distribution over all tweets in dev.}




